Topological charge engineering in lasing bound states in continuum

Recently, optical bound states in continuum in various passive photonic crystals have been identified and similar structures incorporated with optical gain have been reported to exhibit lasing. However, no explicit control over the type of lasing BIC has been reported. In this work, we utilize all four fundamental BICs related to the lowest energy Gamma-point of a square photonic crystal lattice. We identify the associated topological charges from experimentally obtained dispersions, finite element method simulations, as well as from spherical decomposition method based on the microscopic polarization currents in the photonic crystal plane. By tailoring the periodicity and the hole diameter of the photonic crystal slab, we selectively bring each of the four BIC resonances to a wavelength regime, where fluorescent IR702 molecules overlaid with the photonic crystal provide sufficient gain for the onset of lasing. We experimentally analyze all four observed lasing BICs by imaging their far-field polarization vortices and their associated topological charges. The results correspond excellently with the transmission results as well as the simulation results in the absence of gain. Finally, we experimentally present a case where the lasing signal reveals the coexistence of two BICs with opposite topological charges, resulting in a unique polarization pattern. We believe our results enable tailoring the properties, such as polarization winding and topological charge of BICs, by a priori design and thus pave the way for a more general utilization of their appealing properties.

==> extra.tex <==
\subsubsection*{Measurement lasing}
\begin{figure}[H]
\centering
  \subcaptionbox{\label{fig3:a}}{\includegraphics[width=0.4\linewidth]{TM1.png}}\hspace*{1.6em}
  \subcaptionbox{\label{fig3:b}}{\includegraphics[width=0.4\linewidth]{TM2.png}}
  \subcaptionbox{\label{fig3:a}}{\includegraphics[width=.4\linewidth]{TE3.png}}\hspace*{1.6em}
  \subcaptionbox{\label{fig3:b}}{\includegraphics[width=.4\linewidth]{TE4.png}}
\subcaptionbox{\label{fig3:b}}{\includegraphics[width=.4\linewidth]{TWODONUTS.png}}
\caption{\textbf{Lasing measurement in IR-792 environment under unpolarized 780 nm fs laser with 45 degree angle of incidence. The measured energy-spectra shows donut shape( vector beam) near the gamma point, and spatial spectra using WFI shows the polarization rotation of the vector beam when rotating the polarizer clockwise.  } a | p590d360nm . b | p570d460 . c | p570d410nm. d |  p550d300nm. e |  p560d450nm}
\end{figure}
\section{Tommi input}
In Fig b, c, the parameters are p=570 nm,diameters are 410nm,and 460 respectively. By increasing the periodicity by 20 nm and diameter by 80 nm from the previous case,  we increase the gammapoint resonance wavelength of the TE-like modes by approximately 30 nm, and switch the BIC to the low wavelength side TE mode gammapoint (see the red circle). The BIC nature of this mode is verified by the simulations, see xxx. 

A further increase of the diameter to 460 nm induces a BIC to the high wavelength side of the TM mode gammapoint, see the red circles in c, d. Finally,  with parameters p=590nm, d=360nm, we are able to induce a BIC to the low wavelength side of the TM gammapoint. 


\begin{figure}[H]
\centering
  \includegraphics[width=\linewidth]{TE3-VECTOR-OVERALL.PNG}
  \caption{\textbf{Lasing+Multipolar expansion for TM1-p570nm,D460nm.where a) is the lasing measurement obtained from the spectrometer,b) is the polarization map, c) expansion of the dipoles from the multipolar expansion.d) is the intensity profile when taking a horizontal cross section of the donut shape(from the lasing measurement),e) the intensity profile when taking a vertical cross section of the donut shape,f)the intensity profile when summing over the area  the donut shape g)the polarization rotation of the measured lasing beam at 4 different angles, h)radiation pattern obtain from multipolar expansion }}
  \label{vectorTE3}
  \end{figure}


\begin{figure}[H]
\centering
  \includegraphics[width=\linewidth]{TE4-VECTOR-OVERALL.PNG}
  \caption{\textbf{Lasing+Multipolar expansion for TM1-p550nm,D330nm.where a) is the lasing measurement obtained from the spectrometer,b) is the polarization map, c) expansion of the dipoles from the multipolar expansion.d) is the intensity profile when taking a horizontal cross section of the donut shape(from the lasing measurement),e) the intensity profile when taking a vertical cross section of the donut shape,f)the intensity profile when summing over the area  the donut shape g)the polarization rotation of the measured lasing beam at 4 different angles, h)radiation pattern obtain from multipolar expansion }}
  \label{vectorTE4}
  \end{figure}



\begin{figure}
\includegraphics[width=1\columnwidth]{Fig1.jpg}
\caption{test}
\label{fig:Fig2} 
\end{figure}

%{TM2-VECTOR-OVERALL.PNG}
\begin{figure}[H]
\centering
  \includegraphics[width=\linewidth]{lasing-TM2-mode.pdf}
  \caption{\textbf{Lasing+Multipolar expansion for TM1-p570nm,D410nm.where a) is the lasing measurement obtained from the spectrometer,b) is the polarization map, c) expansion of the dipoles from the multipolar expansion.d) is the intensity profile when taking a horizontal cross section of the donut shape(from the lasing measurement),e) the intensity profile when taking a vertical cross section of the donut shape,f)the intensity profile when summing over the area  the donut shape g)the polarization rotation of the measured lasing beam at 4 different angles, h)radiation pattern obtain from multipolar expansion }}
  \label{vectorTM2}
  \end{figure}







